Deep Image Fingerprint: Towards Low Budget Synthetic Image Detection and Model Lineage Analysis

The generation of high-quality images has become widely accessible and is a rapidly evolving process. As a result, anyone can generate images that are indistinguishable from real ones. This leads to a wide range of applications, including malicious usage with deceptive intentions. Despite advances in detection techniques for generated images, a robust detection method still eludes us. Furthermore, model personalization techniques might affect the detection capabilities of existing methods. In this work, we utilize the architectural properties of convolutional neural networks (CNNs) to develop a new detection method. Our method can detect images from a known generative model and enable us to establish relationships between fine-tuned generative models. We tested the method on images produced by both Generative Adversarial Networks (GANs) and recent large text-to-image models (LTIMs) that rely on Diffusion Models. Our approach outperforms others trained under identical conditions and achieves comparable performance to state-of-the-art pre-trained detection methods on images generated by Stable Diffusion and MidJourney, with significantly fewer required train samples.

==> figs/figures/blank_exp.tex <==
\begin{figure}[t]
\captionsetup[subfigure]{labelformat=empty}
\begin{subfigure}{0.3\linewidth}
    \centering
    \vspace{0.65em}
    \begin{minipage}{0.9\textwidth}
        \begin{tikzpicture}[spy using outlines={rectangle,red,magnification=3.5,size=1.5cm, connect spies}]
        \node {\includegraphics[width=1\linewidth,frame]{figs/imgs/blank/target.png}};
        \end{tikzpicture}
        \begin{tikzpicture}[auto]
        \node {\includegraphics[width=1\linewidth,frame]{figs/imgs/blank/targetFFT.png}};
        \end{tikzpicture}
    \end{minipage}
    \caption{Target}
    \end{subfigure}%
     \hfill
    \begin{subfigure}{0.3\linewidth}
    \centering
    \begin{minipage}{0.9\textwidth}
        \begin{tikzpicture}[spy using outlines={rectangle,red,magnification=3.5,size=1.5cm, connect spies}]
        \node {\includegraphics[width=1\linewidth,frame]{figs/imgs/blank/finger_1.png}};
        \tikzset{spy on other={
        \node {\pgfimage[width=1\linewidth]{figs/imgs/blank/finger_1.png}};}}
        \spy on (0.75,-0.5) in node [below] at (0.8,1.5);
        \end{tikzpicture}
        \begin{tikzpicture}[auto]
        \node {\includegraphics[width=1\linewidth,frame]{figs/imgs/blank/fingerFFT_1.png}};
        \end{tikzpicture}
    \end{minipage}
    \caption{$\hat{Y}_a$}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.3\linewidth}
    \centering
    \begin{minipage}{0.9\textwidth}
        \begin{tikzpicture}[spy using outlines={rectangle,red,magnification=3.5,size=1.5cm, connect spies}]
        \node {\includegraphics[width=1\textwidth,frame]{figs/imgs/blank/finger_7.png}};
        \tikzset{spy on other={
        \node {\pgfimage[width=1\textwidth]{figs/imgs/blank/finger_7.png}};}}
        \spy on (0.75,-0.5) in node [below] at (0.8,1.5);
        \end{tikzpicture}
        \begin{tikzpicture}[auto]
        \node {\includegraphics[width=1\textwidth,frame]{figs/imgs/blank/fingerFFT_7.png}};
        \end{tikzpicture}
    \end{minipage}
    \caption{$\hat{Y}_b$}
    \end{subfigure}%
     \caption{
     Result of gray image reconstruction. Left column is a target gray image, whereas center and right columns are results of reconstruction experiments \ohad{the difference is not clear? Are these the result of the same experiment with two different initializations? Something else?}. Bottom row is a \fft{s} of images from top row \ohad{Instead of explaining this in words, add another column to the left, and add the labels ``Image'' and ``FFT'' to it (rotated 90 degrees)}. For $\hat{Y}_a$ and $\hat{Y}_a$ there are also zoomed-in regions of each image \ohad{No need to say there are zoom-ins, it is clear}. \new{Observe pixel noise and its' inconsistency from left to right. These are checkerboard and boundary artifacts respectively.
     \ohad{It's hard to see anything in the zoom-ins. Make the zoom ratio larger, by keeping the zoom-in size the same, but making it show a smaller region of the image.}
     }
     \ohad{The last sentence is not clear. What am I supposed to look at in the figure, and what am I seeing?}
     \ohad{Something is off. The original gray and the reconstructed gray are very different. I refuse to believe that the reconstruction cannot get the correct shade of gray. Maybe there's some normalization somewhere in the process or in the visualization? You'll need to remove it, otherwise it is hard to believe that this ran until convergence.}
     % are hidden within the noise ($\hat{Y}_a$) or clearly visible ($\hat{Y}_b$). In both cases color are inaccurate and \fft{s} are heavily deformed relative an to target.
     }
     \label{fig:monochromeExp}
\end{figure}%


==> figs/figures/blank_expanded.tex <==
\begin{figure*}[t]
\captionsetup[subfigure]{labelformat=empty}
\begin{subfigure}{0.16\linewidth}
    \centering
    \begin{minipage}{0.95\textwidth}
        \begin{tikzpicture}[spy using outlines={rectangle,red,magnification=3.5,size=1.5cm, connect spies}]
        \node {\includegraphics[width=1\linewidth, frame]{figs/imgs/blank/target.png}};
        \end{tikzpicture}
        \begin{tikzpicture}[auto]
        \node {\includegraphics[width=1\linewidth]{figs/imgs/blank/targetFFT.png}};
        \end{tikzpicture}
    \end{minipage}
    \caption{Target}
    \end{subfigure}%
     \hspace{30pt}
    \begin{subfigure}{0.16\linewidth}
    \centering
    \begin{minipage}{0.95\textwidth}
        \begin{tikzpicture}[spy using outlines={rectangle,red,magnification=3.5,size=1.5cm, connect spies}]
        \node {\includegraphics[width=1\linewidth,frame]{figs/imgs/blank_extended/blank10_2000.png}};
        \tikzset{spy on other={
        \node {\pgfimage[width=1\linewidth]{figs/imgs/blank_extended/blank10_2000.png}};}}
        \spy on (0.75,-0.5) in node [below] at (0.8,1.5);
        \end{tikzpicture}
        \begin{tikzpicture}[auto]
        \node {\includegraphics[width=1\linewidth,frame]{figs/imgs/blank_extended/blank10_2000FFT.png}};
        \end{tikzpicture}
    \end{minipage}
    \caption{$\hat{Y}_1$}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.16\linewidth}
    \centering
    \begin{minipage}{0.95\textwidth}
        \begin{tikzpicture}[spy using outlines={rectangle,red,magnification=3.5,size=1.5cm, connect spies}]
        \node {\includegraphics[width=1\linewidth,frame]{figs/imgs/blank_extended/blank19_2000.png}};
        \tikzset{spy on other={
        \node {\pgfimage[width=1\linewidth]{figs/imgs/blank_extended/blank19_2000.png}};}}
        \spy on (0.75,-0.5) in node [below] at (0.8,1.5);
        \end{tikzpicture}
        \begin{tikzpicture}[auto]
        \node {\includegraphics[width=1\linewidth,frame]{figs/imgs/blank_extended/blank19_2000FFT.png}};
        \end{tikzpicture}
    \end{minipage}
    \caption{$\hat{Y}_2$}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.16\linewidth}
    \centering
    \begin{minipage}{0.95\textwidth}
        \begin{tikzpicture}[spy using outlines={rectangle,red,magnification=3.5,size=1.5cm, connect spies}]
        \node {\includegraphics[width=1\linewidth, frame]{figs/imgs/blank_extended/blank33_2000.png}};
        \tikzset{spy on other={
        \node {\pgfimage[width=1\linewidth]{figs/imgs/blank_extended/blank33_2000.png}};}}
        \spy on (0.75,-0.5) in node [below] at (0.8,1.5);
        \end{tikzpicture}
        \begin{tikzpicture}[auto]
        \node {\includegraphics[width=1\linewidth, frame]{figs/imgs/blank_extended/blank33_2000FFT.png}};
        \end{tikzpicture}
    \end{minipage}
    \caption{$\hat{Y}_3$}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.16\linewidth}
    \centering
    \begin{minipage}{0.95\textwidth}
        \begin{tikzpicture}[spy using outlines={rectangle,red,magnification=3.5,size=1.5cm, connect spies}]
        \node {\includegraphics[width=1\textwidth, frame]{figs/imgs/blank_extended/blank4_2000.png}};
        \tikzset{spy on other={
        \node {\pgfimage[width=1\textwidth]{figs/imgs/blank_extended/blank4_2000.png}};}}
        \spy on (0.75,-0.5) in node [below] at (0.8,1.5);
        \end{tikzpicture}
        \begin{tikzpicture}[auto]
        \node {\includegraphics[width=1\textwidth, frame]{figs/imgs/blank_extended/blank4_2000FFT.png}};
        \end{tikzpicture}
    \end{minipage}
    \caption{$\hat{Y}_4$}
    \end{subfigure}%
    
     \caption{Results of gray image reconstruction. Left column is the target gray image, other columns are reconstruction results. Bottom row contains \fft{s} of images from the top row. 
     In all cases, the model produces grid artifacts, i.e. up-sampling and boundary artifacts.
     %For each reconstruction there are also zoomed-in regions of each image.
     }
     \label{fig:monochromeExpand}
\end{figure*}%


==> figs/figures/cross_compare.tex <==
\begin{figure}[t]
    \captionsetup[subfigure]{labelformat=empty}
    \centering
    \begin{subfigure}{0.36\linewidth}
      \includesvg[width=1\linewidth]{figs/imgs/charts/dif_cross.svg}
      \caption{\hspace{0.75cm}DIF}
    \end{subfigure}
    % \hfill
    \begin{subfigure}{0.27\linewidth}
      \includesvg[width=1\linewidth]{figs/imgs/charts/grag_cross.svg}
      \caption{Grag21}
    \end{subfigure}
    % \hfill
    \begin{subfigure}{0.27\linewidth}
    % \includegraphics[width=1.0\linewidth]{figs/imgs/charts/marra_cross.pdf}%
    \includesvg[width=1\linewidth]{figs/imgs/charts/marra_cross.svg}
      \caption{\hspace{-0.5cm}Marra18}
    \end{subfigure}
      \caption{
        Cross-detection accuracy (\%) (DIF, Grag21) and absolute value of cross-correlation (Marra18). The darkest color represent the highest value. The lineage of the models is only observed in the proposed method. The leftmost plot (DIF) is a replication of Figure 5 as a reference.} 
      \label{fig:crossCompare}
    \vspace{-1.5em}
\end{figure}%


==> figs/figures/repeatitions_64_t2i.tex <==
\begin{figure}
    \centering
      \includegraphics[width=\linewidth]{figs/imgs/charts/repeats_64_box.pdf}
      \caption{Accuracy of the train and test repetitions of the DIF per \TI{} as a box plot. Red dots represent reported results from \cref{tab:accuracyTI}.}
      \label{fig:repeats64}
\end{figure}%


==> figs/tables/booter_comparison.tex <==
\begin{table}[ht]
    \centering
    %\small
    \footnotesize
    \begin{tabular}{ lcccccc }
    \toprule 
    \textbf{Loss} & \textbf{SD 1.4} & \textbf{SD 2.1} & \textbf{MJ} & \textbf{\dalM} & \textbf{GLIDE} & \textbf{\dalT} \\
    \midrule
    $\mathcal{L_{B}}, \mathcal{L_{S}}$ & \textbf{99.4} & \textbf{90.7}  & 98.8 & \textbf{99.2} & 90.0 & 79.2 \\
    $\mathcal{L_{S}}$ & 99.3 & 89.5  & \textbf{99.0} & 99.0 & \textbf{90.3} & \textbf{79.5}\\
    $\mathcal{L_{B}}$ & 77.3 & 61.2  & 85.7  & 77.8  & 76.7  & 73.0 \\
    GAN-like & \textbf{99.4} & 89.3  & 98.9  & 99.0  & 89.0  & 78.0 \\
     \bottomrule 
    \end{tabular}
    \caption{Detection accuracy (\%) on \TI{} images.
    ${\mathcal{L_{B}}}$ and ${\mathcal{L_{S}}}$ refer to the application of the Booster loss and Sample loss, respectively. GAN-like denotes a decoder-only model trained with ${\mathcal{L_{S}}}$. Train set contains 1024 images.
    \label{tab:accuracyBoost}}
    \vspace{-2.5em}
\end{table}

==> figs/tables/comparison.tex <==

\begin{table*}[ht]
    \centering
    \small
    \begin{tabular}{ llcccccc }
    \toprule 
    \textbf{$N_S$} &\textbf{Method} & \textbf{SD 1.4} & \textbf{SD 2.1} & \textbf{MJ} &\textbf{\dalM}&\textbf{GLIDE} & \textbf{\dalT}\\
    \midrule
    \multirow{2}{2.em}{1024} & DIF$_{\mathcal{L_{B}}}$ & \textbf{99.4} & \textbf{90.7}  & 98.8 & \textbf{99.2} & 90.0 & 79.2 \\
    & DIF & 99.3 & 89.5  & \textbf{99.0} & 99.0 & \textbf{90.3} & \textbf{79.5}\\
    \midrule
    
    \multirow{2}{2.em}{512} &  DIF$_{\mathcal{L_{B}}}$ & 98.9 & \textbf{88.5}  & \textbf{99.0} & 98.6 & 87.9 & \textbf{79.6}  \\
    & DIF & \textbf{99.2} & 86.3  & 98.8 & \textbf{98.7} & \textbf{88.2} & 79.1 \\
    \midrule
    
    \multirow{2}{2.em}{256} & DIF$_{\mathcal{L_{B}}}$ & 98.2 & \textbf{81.5}  & \textbf{98.4} & 97.7 & 85.5 & 76.9\\
    & DIF & \textbf{98.5} & 81.3  & 98.1 & \textbf{98.0} & \textbf{85.9} & \textbf{77.7}\\
    \midrule
    
    \multirow{2}{2.em}{128} & DIF$_{\mathcal{L_{B}}}$& \textbf{97.9} & 74.9  & 97.2 & 96.7 & 79.5 & \textbf{78.0}\\
    & DIF & 97.7 & \textbf{75.5}  & \textbf{97.3} & \textbf{97.0} & 81.4 & 76.1\\
     \bottomrule 
    \end{tabular}
    \caption{Detection accuracy (\%) of the proposed method on images from \TI{s}. ${\mathcal{L_{B}}}$ denotes when Booster loss and augmentations are used. 
    \label{tab:accuracyDIFs}}
\end{table*}


==> figs/tables/comparisonTI.tex <==

% Comparison of proposed method to others

\begin{table*}[ht]
    \centering
    \footnotesize
    \begin{tabular}{ llcccccc|c }
    \toprule 
    \textbf{$N_S$} &\textbf{Method} & \textbf{SD 1.4} & \textbf{SD 2.1} & \textbf{MJ} &\textbf{\dalM}& \textbf{GLIDE} & \textbf{\dalT} & \textbf{Mean}\\
    \midrule
    \multirow{9}{2.em}{1024} & Joslin20  & 49.7 & 49.9  & 49.9 & 52.3 & 57.0 & 51.4 & 51.7 \\
    & Marra18 & 52.6 & 48.0  & 75.7 & 85.3 & 57.6 & 56.3 & 62.6  \\
    & Ning18 & 50.8 & 51.4  & 59.5 & 58.1 & 57.7 & 52.2 & 55.0 \\
    & Wang20$_{F}$ &  63.7 & 61.7 & 75.7 & 78.3 & 74.5 & 74.7 & 71.4  \\
    & Resnet50$_{F}$ & 72.2 & 72.6 & 87.1 & 87.5 & 94.1 & 88.7 & 83.7  \\
    & Grag21 &  69.2 & 73.6 & 89.7 & 89.4 & 94.3 & 85.9  & 83.7 \\
    & Grag21$_{F}$ & 93.5 & 86.9 & 93.5 & 96.1 & \textbf{97.5} & \textbf{93.5}  & 93.5 \\
   & Corv22$_{F}$ &  \textbf{99.7} & \textbf{99.0} & \textbf{99.2} & 96.4 & 96.0 & 91.9  & \textbf{97.0} \\
    & DIF & 99.3 & 89.5  & 99.0 & \textbf{99.0} & 90.3 & 79.5  & \underline{92.8} \\
    \midrule
    
    \multirow{5}{2.em}{512} & Resnet50$_{F}$ & 70.6 & 70.5 & 90.0 & 85.4 & 92.7 & 85.4  & 82.4 \\
    & Grag21 &  68.3 & 71.4 & 81.1 & 85.2 & 91.3 & 83.8 & 80.2  \\
    & Grag21$_{F}$  &  93.0 & 86.0 & 94.7 & 96.1 & \textbf{96.4} & \textbf{92.1}  & 93.1  \\
    & Corv22$_{F}$ &  \textbf{99.6} & \textbf{98.6} & \textbf{98.8} & 95.9 & 95.1 & 89.4  &\textbf{96.2} \\
    & DIF & 99.2 & 86.3  & \textbf{98.8} & \textbf{98.7} & 88.2 & 79.1  & \underline{91.7} \\
    \midrule
    
    \multirow{5}{2.em}{256} & Resnet50$_{F}$ & 66.2 & 64.0 & 86.4 & 82.0 & 89.0 & 81.4  & 78.2  \\
    & Grag21 &  67.2 & 65.8 & 74.4 &  83.5 & 88.0 & 75.3  & 75.7 \\
    & Grag21$_{F}$  &  89.9 & 82.9 & 94.1 & 94.9 & \textbf{95.6} & 90.5  & 91.3 \\
    & Corv22$_{F}$ &  \textbf{99.6} & \textbf{98.6} & \textbf{99.0} & 95.6 & 94.8 & 89.0  & \textbf{96.1} \\
    & DIF & 98.5 & 81.3  & 98.1 & \textbf{98.0} & 85.9 & 77.7  & \underline{89.9} \\
    \midrule
    
    \multirow{5}{2.em}{128} & Resnet50$_{F}$ & 66.2 & 64.0 & 85.9 & 75.1 & 87.6 & 75.2  & 75.7 \\
    & Grag21 &  68.0 & 66.4 & 72.6 & 81.0 & 80.3 & 71.7  & 73.3\\
    & Grag21$_{F}$  &  87.9 & 82.2 & 93.4 & 93.5 & \textbf{94.2} & \textbf{90.4}  & 90.3 \\
    & Corv22$_{F}$ &  \textbf{99.6} & \textbf{98.4} & \textbf{98.6} & 93.9 & 89.1 & 77.5 & \textbf{92.9} \\
    & DIF & 97.7 & 75.5  & 97.3 & \textbf{97.0} & 81.4 & 76.1  & \underline{87.5} \\
    \midrule
    
    \multirow{3}{2.em}{---}& Wang20$_{D}$ &  50.0 & 49.8 & 50.2 & 50.7 & 53.3 & 51.0  & 55.9 \\
    & Grag21$_{D}$ &  57.0 & 50.2 & 63.1 & 58.0 & 54.3 & 51.2  & 55.6 \\
    & Corv22$_{D}$ &  \textbf{99.3} & \textbf{99.3} & \textbf{99.0} & \textbf{89.5} & \textbf{57.0} & \textbf{51.6}  & \textbf{82.6} \\
     \bottomrule
     
    \end{tabular}
    \caption{Classification accuracy (\%). $N_S$ is the amount of train samples. Methods are indexed as follows: $D$ pre-trained and not fine-tuned, $F$ pre-trained and fine-tuned on the given data, no index indicates that the model is trained from scratch. \new{The only true competitor to DIF are fine-tuned SOTA Grag21 and Corv22, which were pre trained on a large datasets. Corv22 is expected to have edge over DIF as it was pre-trained on images from SD models. \serge{If we leave Grag22 then we should remove one of the $N_S$ sections.}}
    \label{tab:accuracyTI}}
\end{table*}


==> figs/tables/gan_test.tex <==

% \begin{table}[ht]
%     \centering
%     \small
%     \begin{tabular}{ lcccc }
%     \toprule 
%     \textbf{Image Class} & w/o $\mathcal{L_{B}}$, $\alpha = 1.0$ & w $\mathcal{L_{B}}, \alpha = 0.5$ & DnCNN, $\mathcal{L_{B}}, \alpha = 0.5$ & w/o $\mathcal{L_{B}}$, DnCNN \\
%     \midrule
%     BigGAN & \textbf{98.2}  & 97.3 & 96.8 & 96.9 \\
%     CycleGAN & \textbf{96.4}  & 95.4 & 92.4 & 94.4 \\
%     GauGAN & 88.1  & 92.2 & \textbf{92.6} & 91.8  \\
%     StarGAN & 99.5 & \textbf{99.9} &  99.8 & \textbf{99.9}  \\
%     StyleGAN & \textbf{99.7} & 93.0 & 96.1 & 96.6 \\
%     StyleGAN2 &  \textbf{93.2} & 85.4 & 92.0 & 91.5  \\
%     ProGAN &  56.6 & 61.6 & \textbf{67.1} &  57.6  \\
%     \midrule
%     Mean &  91.2 & 75.0 & \textbf{91.3} & 89.8  \\
%     \bottomrule
%     \end{tabular}
%     \caption{Accuracy of a DIF by GAN models image classes in percents. \\
%     \label{tab:gans}}
% \end{table}

\begin{table}[ht]
    \centering
    \small
    \begin{tabular}{ lcc }
    \toprule 
    \textbf{GAN Model} & $\mathcal{L_{B}}$ & w/o $\mathcal{L_{B}}$\\
    \midrule
    BigGAN  & 96.8 & \textbf{96.9} \\
    CycleGAN  & 92.4 & \textbf{94.4} \\
    GauGAN  & \textbf{92.6} & 91.8  \\
    StarGAN &  99.8 & \textbf{99.9}  \\
    StyleGAN & 96.1 & \textbf{96.6} \\
    StyleGAN2 & \textbf{92.0} & 91.5  \\
    ProGAN$_e$ & \textbf{67.1} &  57.6  \\
    \bottomrule
    \end{tabular}
    \caption{Accuracy (\%) for images generated by GAN models. Usage of $\mathcal{L_{B}}$ implies augmentations during the training.
    \label{tab:gans}}
\end{table}


==> figs/tables/progran.tex <==

% Comparison of proposed method to others

\begin{table}[ht]
    \centering
    \small
    \begin{tabular}{ lccc }
    \toprule 
    \textbf{Image Class} & w/o $\mathcal{L_{B}}$ & w $\mathcal{L_{B}}$ & DnCNN w/o $\mathcal{L_{B}}$\\\\
    \midrule
    airplane & 86.5  & 85.8 & \textbf{91.1}  \\
    bicycle & 86.1  & \textbf{90.5} & 90.2  \\
    bird & 87.4  & 89.4 & \textbf{92.1}  \\
    boat & 89.2  & 91.4 & \textbf{92.9} \\
    bottle &  \textbf{83.6}  & 82.6 & 83.2  \\
    bus & 89.1  & 88.6 & \textbf{90.0} \\
    car & 88.1  & 90.9 & \textbf{91.1}  \\
    cat & 93.7  & 93.7 & \textbf{94.1}  \\
    chair & 83.3  & 84.8 & \textbf{91.1}  \\
    cow & 93.9  & 94.6 & \textbf{94.8} \\
    diningtable & 88.3  & 93.1 & \textbf{96.0}  \\
    dog & 92.7  & \textbf{94.3} & 94.1  \\
    horse & 91.1  & 93.2 & \textbf{95.0}  \\
    motorbike & 81.0  & 82.6 & \textbf{85.7} \\
    person & 82.2  & 86.2 & \textbf{90.5}  \\
    pottedplant & 89.3  & 90.7 &  \textbf{90.8}  \\
    sheep & 95.8   & \textbf{96.2} & 95.7 \\
    sofa & 85.0  & 90.2 & \textbf{93.2} \\
    train & 86.6 & 85.7 & \textbf{88.2} \\
    tvmonitor & 74.7  & 74.8 & \textbf{83.6} \\
    \midrule
    Mean & 87.4  & 89.0 & \textbf{91.2} \\
    \bottomrule
    \end{tabular}
    \caption{Accuracy of a DIF by ProGAN image classes in percents. \\
    \label{tab:progan}}
\end{table}


==> macros.tex <==
\newcommand{\betweencellpdf}{\ensuremath{h^c}}
\newcommand{\betweencellpdffine}{\ensuremath{h^f}}
\newcommand{\approxbetweencellpdffine}{\ensuremath{\hat{h}^f}}
\newcommand{\incellpdf}{\ensuremath{f}}
\newcommand{\incellpdfnormalized}{\ensuremath{f'}}

\newcommand{\incellcdf}{\ensuremath{F}}

\newcommand{\totalpdf}{\ensuremath{f_{dd}}}
\newcommand{\totalcdf}{\ensuremath{F_{dd}}}

\newcommand{\ignorethis}[1]{}
\newcommand{\redund}[1]{#1}

% \newcommand{\etal       }     {{et~al.}}
\newcommand{\apriori    }     {\textit{a~priori}}
\newcommand{\aposteriori}     {\textit{a~posteriori}}
\newcommand{\perse      }     {\textit{per~se}}
% \newcommand{\eg         }     {{e.g.}}
% \newcommand{\Eg         }     {{E.g.}}
% \newcommand{\ie         }     {{i.e.}}
\newcommand{\naive      }     {{na\"{\i}ve}}
\newcommand{\Naive      }     {{Na\"{\i}ve}}
\newcommand{\Identity   }     {\mat{I}}
\newcommand{\Zero       }     {\mathbf{0}}
\newcommand{\Reals      }     {{\textrm{I\kern-0.18em R}}}
\newcommand{\isdefined  }     {\mbox{\hspace{0.5ex}:=\hspace{0.5ex}}}
\newcommand{\texthalf   }     {\ensuremath{\textstyle\frac{1}{2}}}
\newcommand{\half       }     {\ensuremath{\frac{1}{2}}}
\newcommand{\third      }     {\ensuremath{\frac{1}{3}}}
\newcommand{\fourth     }     {\ensuremath{\frac{1}{4}}}

\newcommand{\Lone} {\ensuremath{L_1}}
\newcommand{\Ltwo} {\ensuremath{L_2}}

\newcommand{\degree} {\ensuremath{^{\circ}}}

\newcommand{\mat        } [1] {{\text{\boldmath $\mathbit{#1}$}}}
\newcommand{\Approx     } [1] {\widetilde{#1}}
\newcommand{\change     } [1] {\mbox{{\footnotesize $\Delta$} \kern-3pt}#1}

\newcommand{\Order      } [1] {O(#1)}
\newcommand{\set        } [1] {{\lbrace #1 \rbrace}}
\newcommand{\floor      } [1] {{\lfloor #1 \rfloor}}
\newcommand{\ceil       } [1] {{\lceil  #1 \rceil }}
\newcommand{\inverse    } [1] {{#1}^{-1}}
\newcommand{\transpose  } [1] {{#1}^\mathrm{T}}
\newcommand{\invtransp  } [1] {{#1}^{-\mathrm{T}}}
\newcommand{\relu       } [1] {{\lbrack #1 \rbrack_+}}

\newcommand{\abs        } [1] {{| #1 |}}
\newcommand{\Abs        } [1] {{\left| #1 \right|}}
\newcommand{\norm       } [1] {{\| #1 \|}}
\newcommand{\Norm       } [1] {{\left\| #1 \right\|}}
\newcommand{\pnorm      } [2] {\norm{#1}_{#2}}
\newcommand{\Pnorm      } [2] {\Norm{#1}_{#2}}
\newcommand{\inner      } [2] {{\langle {#1} \, | \, {#2} \rangle}}
\newcommand{\Inner      } [2] {{\left\langle \begin{array}{@{}c|c@{}}
                               \displaystyle {#1} & \displaystyle {#2}
                               \end{array} \right\rangle}}

\newcommand{\twopartdef}[4]
{
  \left\{
  \begin{array}{ll}
    #1 & \mbox{if } #2 \\
    #3 & \mbox{if } #4
  \end{array}
  \right.
}

\newcommand{\fourpartdef}[8]
{
  \left\{
  \begin{array}{ll}
    #1 & \mbox{if } #2 \\
    #3 & \mbox{if } #4 \\
    #5 & \mbox{if } #6 \\
    #7 & \mbox{if } #8
  \end{array}
  \right.
}

\newcommand{\len}[1]{\text{len}(#1)}



\newlength{\w}
\newlength{\h}
\newlength{\x}

\definecolor{darkred}{rgb}{0.7,0.1,0.1}
\definecolor{darkgreen}{rgb}{0.1,0.6,0.1}
\definecolor{cyan}{rgb}{0.7,0.0,0.7}
\definecolor{otherblue}{rgb}{0.1,0.4,0.8}
\definecolor{maroon}{rgb}{0.76,.13,.28}
\definecolor{burntorange}{rgb}{0.81,.33,0}

\ifdefined\ShowNotes
  \newcommand{\colornote}[3]{{\color{#1}\textbf{#2} #3\normalfont}}
\else
  \newcommand{\colornote}[3]{}
\fi

%\newcommand {\note}[1]{\colornote{maroon}{}{#1}}
\newcommand {\todo}[1]{\colornote{cyan}{TODO}{#1}}
\newcommand {\ohad}[1]{\colornote{cyan}{OF:}{#1}}
\newcommand {\serge}[1]{\colornote{darkgreen}{SS:}{#1}}

\newcommand {\reqs}[1]{\colornote{red}{\tiny #1}}

\ifdefined\ShowNewNotes
  \newcommand{\colornewnote}[1]{{\color{red}#1\normalfont}}
\else
  \newcommand{\colornewnote}[1]{#1}
\fi

\newcommand {\new}[1]{{\colornewnote{#1}}}

\newcommand*\rot[1]{\rotatebox{90}{#1}}

\newcommand {\newstuff}[1]{#1}

\newcommand\todosilent[1]{}


\newcommand{\woBGmask}{{w/o~bg~\&~mask}}
\newcommand{\woMask}{{w/o~mask}}

% Keywords command
\providecommand{\keywords}[1]
{
  %\small	
  \textbf{\textit{Keywords---}} #1
}

%\newcommand {\shortcite}[1]{\cite{#1}}

%\newcommand {\paragraph}[1]{\noindent\textbf{#1}}


